On the Costs and Benefits of Adopting Lifelong Learning for Software Analytics -- Empirical Study on Brown Build and Risk Prediction

Nowadays, software analytics tools using machine learning (ML) models to, for example, predict the risk of a code change are well established. However, as the goals of a project shift over time, and developers and their habits change, the performance of said models tends to degrade (drift) over time. Current retraining practices typically require retraining a new model from scratch on a large updated dataset when performance decay is observed, thus incurring a computational cost; also there is no continuity between the models as the past model is discarded and ignored during the new model training. Even though the literature has taken interest in online learning approaches, those have rarely been integrated and evaluated in industrial environments. This paper evaluates the use of lifelong learning (LL) for industrial use cases at Ubisoft, evaluating both the performance and the required computational effort in comparison to the retraining-from-scratch approaches commonly used by the industry. LL is used to continuously build and maintain ML-based software analytics tools using an incremental learner that progressively updates the old model using new data. To avoid so-called "catastrophic forgetting" of important older data points, we adopt a replay buffer of older data, which still allows us to drastically reduce the size of the overall training dataset, and hence model training time.

==> content/old_files/RQ0.tex <==

\input{tables/RQ0}

\subsection{Preliminary study: MLP architecture tuning}

\subsubsection{Approach}

This section aims at finding the best architecture for an MLP for our use cases.
Each combination of hyperparameters considered (\ie learning rate, number of layers and size of the layers) was run four times, using a cross-validation setup (80-10-10\% for training-validation-test) run in 5 different folds. We report the results of predictions on the test set for the best model architecture based on median validation performance. 
% Each cross-validation randomly splits the data into 5 folds, which are themselves split in 2 sub-folds. The sub-folds of a given fold each become the validation set once, and the test set once, amounting to 10 different training, validation and test sets, where the validation set is used for hyperparameter tuning, while the model's performance is assessed on the test set. We repeat the 5-fold cross-validation 4 times (40 experiments). 


For the brown build detection use case, we compare to an XGBoost-based model similar to our industry partner's model. For JIT risk prediction, we compare to the AlwaysRisky baseline.
At this point, the subset split does not respect the timeline of jobs and that the subsets are split randomly, \ie we are not yet using LL or RFS in this preliminary study. %


\subsubsection{Results}

\textbf{For the studied brown build projects, the F1-score of using an MLP with cross-validation setup is close, if not higher than the F1-score of the XGboost model (from -2\% to +11\%), and 3-9 times higher than the best intuitive baseline AlwaysBrown; for the JIT risk use case it is 1.6-2.4 times higher than AlwaysRisky.}
In Table~\ref{MLP_hyper_res}, we observe that the MLP model has a higher F1-score than the XGBoost model for projects Brown\_1 (+11\%),  Brown\_2 (+3\%) and  Brown\_3 (+8\%), while it performs 2\% lower for project Brown\_OSS's F1-score. However, the F1-score is still four times higher than an intuitive baseline (AlwaysBrown).
In terms of G-mean, MLP again performs better than XGBoost for 3 out of 4 projects, with slight changes compared to the F1-score results.

For JIT risk prediction, the F1-score varies from 21-49\%, which are the best average results obtained for each given project's 4 runs. 
For this use case, we did not have access to the original XGBoost-based model used by our industrial partner, so we compare the results only to AlwaysRisky. 
The MLP model's F1-score performs 1.6-2.4 times better than AlwaysRisky regarding the F1-score.

==> content/old_files/intro.tex <==
Software analytics models, and the tools built on them, rarely take into account the drifting nature of software engineering data when training and deploying.
Researchers have introduced a wide range of analytics tools for build failure prediction in Continuous Integration (CI)~\cite{saidani2022improving}, test case prioritization~\cite{marijan2022comparative}, code recommendation~\cite{luan2019aroma, schumacher2020improving}, amongst others.
While such models might work accurately right after training, their predictions tend to become outdated over time as they are being used in production~\cite{ekanayake2009tracking}. 
MLOps engineers refer to this phenomenon of model and dataset aging as ``concept drift''~\cite{sato2019continuous,gift2021practical,lu2018learning}. The term ``concept'' refers to a segment of a dataset along a timeline with a given data distribution, and drift refers to the transition between concepts.

Concept drift implies that models trained on older segments of data no longer provide information relevant to the prediction in the current segment, potentially harming the performance of the model in production~\cite{gama2014survey}. The best developers can do is to manually retrain a model and re-release the tool with the updated model, yet this requires them to decide when to retrain and what training data to use. Such retraining-from-scratch (RFS) typically requires a large data set (making retraining slower~\cite{tsangaratos2016comparison, chen2016xgboost, chung2008minimum}), and ignores prior models' knowledge, which goes against traditional software re-engineering practices~\cite{demeyer2002object}. 

To intrinsically deal with concept drift, the domain of machine learning has been exploring online learning approaches. 
Online learning covers various paradigms that attempt at mimicking the human ability to retrain and accumulate knowledge previously learned~\cite{liu2017lifelong}.
In the context of software analytics, prior work incrementally updates the training data with new incoming data, considering resampling approaches to deal with data imbalance~\cite{mcintosh2018fix,tan2015online}.
\Do{new=>}Works have studied online learning setups based on bagging approaches, where neural networks are bagged and updated over time with new data points only~\cite{cabral2019class,tabassum2020investigation,cabral2022towards} and approaches using memory-based updates~\cite{gao2023keeping}. 

Such online approaches come with many challenges in practice, and have thus rarely been introduced in industrial settings~\cite{barry2023streamai}.
Industrial settings are constrained by efficiency, where resources for ML training might be limited.

This paper focuses on applying to industrial projects the paradigm of online learning called ``Lifelong learning'' (LL)~\cite{parisi2019continual} and evaluating the advantage of such approach regarding maintenance effort.
The approach we use incrementally updates one given model using both recent and older data (replay buffer). 
LL setups use incremental learning models such as Neural Networks (NN), similarly to Cabral et al.'s approach~\cite{cabral2019class}, but with an addition of a memory-based mechanism inspired by Gao et al.~\cite{gao2023keeping}.  
In online setups, including LL, model updates can also be performed more often, since the computation time of LL retraining is smaller than for RFS.
\Do{<=end}

We study the degree to which an LL setup enables faster incremental evolution of a deployed model to deal with drift during operations compared to retraining from scratch.
Our empirical study focuses on two typical software analytics use cases, brown build detection and Just-In-Time (JIT) risk prediction. Brown build detection is related to flaky test analysis, which is one of the emerging topics in software testing in recent years~\cite{olewicki2022towards, bell2018deflaker, alshammari2021flakeflagger}. JIT risk prediction is a generalization of bug prediction models, a staple of software analytics for 20 years, that focuses on the overall risk (e.g., test failure, code complexity) of a change. Both use cases have been adopted in some form by our industry partner, showing signs of concept drift.
Through empirical evaluation on a total of eight large projects, seven from our industrial collaborator and one open-source, we address the following research questions:


\textbf{RQ1: \RQone} 
Comparison with different RFS setups for the two use cases currently used by our industrial partner shows that the LL setup significantly outperforms the currently used approaches \num{(+9-31\% F1 score) for 6 out of the 8 studied projects (large effect size), and behaves similarly in the other 2 projects.
We also find that it performs similarly to an NN-based RFS setup in 4/8 cases, better in 3/8 cases and significantly worse in 1/8 case.}

\textbf{RQ2: \RQtwo} 
A major issue encountered with LL setups is catastrophic forgetting, where, during updating, the model forgets previously acquired knowledge.  
To address this, we adopt a memory-based approach that trains the model with additional samples of past data points. 
\num{We observe that this approach improves significantly the F1-score compared to a more naive LL setup (+4-26\%) for 3/8 cases, while not showing significant differences in the other 5 cases (-1\% to +6\%).}

\textbf{RQ3: \RQthree} 
We compare the computational effort needed to perform LL updates with RFS. Even though the LL setup needs 1.1-8.75 times more updates, the LL updates are computationally less expensive since 3.3-13.7 times less data is necessary for retraining, on average.

Finally, we discuss trade-offs in terms of the training setups' flexibility to adjust to drift versus continuity of the models' human interpretation. 


==> content/old_files/methodology.tex <==


\begin{table*}[t]
    \centering
    \caption{Cross-validation performance of hyperparameter optimization for the MLP models for the brown build detection and JIT risk prediction use cases. (For brown build detection, the \textcolor{cyan}{\textbf{bolded blue}} values show the best F1-score per project.)}
    \label{MLP_hyper_res}
    \begin{tabular}{|l|ccccc|ccccc|ccccc|ccccc|}
        \hline
         \multirow{3}{*}{Model}& \multicolumn{5}{c|}{Project Brown\_1} 
         & \multicolumn{5}{c|}{Project Brown\_2} 
         & \multicolumn{5}{c|}{Project Brown\_3} 
         & \multicolumn{5}{c|}{Project Brown\_OSS} \\ \cline{2-21}
         &\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}
         &\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}
         &\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}
         &\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}\\
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec\\ \hline
    	
    AlwaysBrown&
        23&30&100&na&0&
		27&37&100&na&0&
		5&5&100&na&0&
		12&13&100&na&0\\
% 	\textit{Random50}&
%         19&30&50&70&50&
% 		21&37&50&63&50&
% 		5&5&50&95&50&
% 		10&13&50&87&50\\
% 	\textit{RandomB}&
%         15&30&30&70&70&
% 		19&37&37&63&63&
% 		3&5&5&95&95&
% 		6&13&13&87&87\\
       XGBoost&62&55&72&86&75 &67&57&81&85&64 &36&35&38&97&96 &\textcolor{cyan}{\textbf{52}}&{47}&{57}&{91}&{91}\\
    NN  &\textcolor{cyan}{\textbf{73}}&{64}&{85}&{90}&{73}
        &\textcolor{cyan}{\textbf{70}}&{66}&{75}&{77}&{67}
        &\textcolor{cyan}{\textbf{44}}&{35}&{61}&{89}&{75}
        &50&38&73&95&81\\
    \hline
     \hline
         \multirow{3}{*}{Model}& \multicolumn{5}{c|}{Project Risk\_1} 
         & \multicolumn{5}{c|}{Project Risk\_2} 
         & \multicolumn{5}{c|}{Project Risk\_3} 
         & \multicolumn{5}{c|}{Project Risk\_4} \\ \cline{2-21}
         &\multicolumn{3}{c|}{Risk}&\multicolumn{2}{c|}{Safe}
         &\multicolumn{3}{c|}{Risk}&\multicolumn{2}{c|}{Safe}
         &\multicolumn{3}{c|}{Risk}&\multicolumn{2}{c|}{Safe}
         &\multicolumn{3}{c|}{Risk}&\multicolumn{2}{c|}{Safe}\\
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec
         &F1&Pre&\multicolumn{1}{c|}{Rec}&Pre&Rec\\ \hline
    AlwaysRisky&
        19&24   &100&na&0&
		21&27   &100&na&0&
		19&24    &100&na&0&
		13&15   &100&na&0\\
    NN  & 45& 67& 36& 81& 93
        & 49& 63& 42& 78& 90
        & 43& 63& 36& 82& 93
        & 21& 38& 15& 92& 98\\ 
    \hline
    \end{tabular}

\end{table*}

\subsection{Multi-layer perceptron neural networks} \label{sec:MLP}

An LL setup requires an incremental learning algorithm, such as multi-layer perceptron (MLP) neural networks, which are retrained in a specific manner. This section first discusses the basic MLP training process and the methodology used to tune hyperparameters. The next sections detail the use of MLPs in an LL setup.

\subsubsection{MLP training process}

A basic MLP has $L$ layers of size $N$. After each hidden-layer, except the last one, an activation function (e.g., ReLU\footnote{Torch ReLU activation function: \url{https://pytorch.org/docs/stable/generated/torch.nn.ReLU.html}}) is applied to the last layer before in is inputed to the next layer. After the last layer, a sigmoid activation function\footnote{Torch sigmoid activation function: \url{https://pytorch.org/docs/stable/generated/torch.nn.Sigmoid.html}} is applied to bound the final output values between $[0;1]$ (i.e., obtain probabilities as output). Algorithm~\ref{algo_nn} shows the pseudo-code for a typical MLP training process. In essence, in each iteration (``epoch'') the training algorithm compares the output of the current model on subsets (``minibatch'') of the training set to the expected output, then tries to minimize the resulting ``loss'' using an optimizer. It is clear how the complexity of this algorithm is linearly dependent on the number of epochs and the size of the training set (divided by the size of a minibatch).

Implementation-wise, the loss function we used is Binary Cross Entropy, while the optimizer we consider is Adam (with hyperparameter learning rate $lr$). 
Both were chosen after preliminary evaluation instead of, respectivelythe loss functions Mean Squared Error (MSE) and Mean Absolute Error (MAE), and the optimizer Stochastic Gradient Descent (SGD).
The MLP training is done using minibatch\cite{li2014efficient}, with minibatches of size 20 and with 50 epochs at each training.


\begin{algorithm}[t]
\caption{Pseudo-code for training of an NN.}\label{algo_nn}
\begin{algorithmic}
\REQUIRE{trainset with dataset "X" and labels "y", NN, epoch}
\FOR{iter in epoch}
 \STATE Split trainset in minibatches
 \FOR{minibatch in trainset}
 \STATE pred = NN(minibatch[X]) //model's outputs on minibatch
 \STATE loss = lossfun(minibatch[y], pred) //loss versus labeled data
 \STATE net.update(optimizer(NN, loss)) //update model weights
 \ENDFOR
 \ENDFOR
% \ENSURE{bobo}
\end{algorithmic}
\end{algorithm}


\subsubsection{Hyperparameter tuning approach}

This section aims at finding the best architecture for an MLP in the context of our use cases.
% The different hyperparameters values we considered for the NN architecture optimization are gathered in Table~\ref{brown:hyper_val} in the MLP category. 
Each combination of hyperparameters considered (i.e., learning rate, number of layers and size of the layers) was run four times, using a cross-validation set-up (80\% training, 10\% validation, and 10\% test).
Note that, at this point, the subset split does not respect the timeline of jobs and the subsets are split randomly. In later sections, we will focus on actual prediction. For the brown build detection use case, we had access to an XGBoost-based model used by our industry partner, which we use as baseline for tuning.

\subsubsection{Hyperparameter tuning results}
\textbf{For the studied brown build projects, the F1-score of using an MLP with cross validation setup is close, if not higher than the F1-score of the XGboost model (between -2\% and +11\%) and 3 to 9 times higher than the best intuitive baseline \textit{AlwaysBrown}.}

In Table~\ref{MLP_hyper_res}, %shows the results for each project for the Brown Build detection use case.
% The best hyper-parameters chosen are indicated in Table~\ref{brown:hyper_val}.
we observe that the MLP model performs better than the XGBoost model for projects Brown\_1 (+11\%),  Brown\_2 (+3\%) and  Brown\_3 (+8\%) in terms of F1-score, while it performs 2\% lower for project Brown\_OSS's F1-score% is 50\% which is 2\% lower than XGBoost models
. However, the F1-score is still four times higher than an intuitive baseline that would always return ``Brown'' as a prediction (AlwaysBrown).



For the JIT risk prediction use case, %we also did cross-validation to define the best NN architecture. The results are shown in Table~\ref{MLP_hyper_res}. When considering the F1 score, 
we can see how the results vary from 21-49\%, which are the average best results obtained for each given project's four runs. 
For this use case, we did not have access to original XGBoost-based model used by our industrial partner, so we compare the results only to an intuitive baseline (AlwaysRisky), that always predict code changes to be risky. 
The NN model performs 1.3 to 2.4 times better than AlwaysRisky.


\subsection{Data splitting} 

In an actual production environment, the datasets used for models are split chronologically such that the training, validation, and test sets do not overlap. Furthermore, in the case of brown build detection, to reduce information contamination among build jobs from a same commit, all the jobs allocated to a given commit always appear in the same subset.

In a lifelong learning setup, the dataset is split into successive ``time groups''. Groups are split according to the number of consecutive commits encountered, the group size $GS$ being a hyperparameter of the setup. The split is not done according to a time period to maintain a consistent amount of data in each group, since software engineering datasets have varying activity over time, with some weeks having little to no data points. This is for example an issue for projects with low $\beta$ in the case of brown build detection or projects with low $RR$ in the case of JIT risk prediction. Furthermore, in an LL setup, each model update needs to train on time groups with a decent amount of data in order not to overfit to new data points and not to unlearn brown/risk prediction because of sparse training sets. % not containing any. %to have a consistent number of data points in each sub-dataset. 
Note that for the brown build detection use case the choice for a fixed number of commits per group implies that the size of the groups may vary depending on how many builds were triggered for each commit.
  

\subsection{Lifelong learning training process}


\begin{figure}[t]
	\centering
	\includegraphics[width=.49\textwidth]{img/CL_setup}
	\caption{Lifelong learning set-up\label{fig:LL_setup}. The validation set is a sliding window of size $VWin=3$, while the initial training window size $ITWin=3$ and the replay buffer window size $RBWin=3$.}
\end{figure}

\subsubsection{Overall algorithm}

At each time step of the LL training process, the algorithm shifts up one time group of data, then defines separate sub-datasets for training, validation, and testing of the NN model. In Figure~\ref{fig:LL_setup}, we can see the first 3 time steps (named ``Initialization'', ``Update1'' and ``Update2'') of an LL setup, each having a sliding window validation set of size $VWin=3$ (as an example), and training/test sub-datasets of 1 time group each.

A given time step's three sub-datasets do not overlap amongst each other; similarly, even though a given time group is used for the training, validation and/or test sets of different time steps, the data sampled within those groups does not overlap. For example, group 2's data is used in the Train1/Valid1 data sets of the Initialization step, and the Valid2 data set of the Update1 step, however the intersection of those data sets is empty. Note that Train1 covers $VWin$ groups, while the update steps' Train2/Train3 only cover 1 group, because even when using LL the initial model has to be trained from scratch, only model updates can benefit of LL.%Essentially, %same periods on the timeline but the data itself does not overlap. Each data point will appear in at most one of the sets (training, validation or test) at each training step. T
%the validation set works as a sliding window of size $VWin$ selecting consecutive groups. 

In addition to those sets, we define a replay buffer, which is used to limit the catastrophic forgetting of the model. 
The replay buffer is built as we go through the different time steps, by randomly selecting a portion of the new training data points %(the training set on Figure~\ref{fig:LL_setup} 
found since the last update.
That sample is balanced, i.e., the same number of data points is selected of each classification label.
%At each step, new data points are added from the current training set to the replay buffer. 
As mentioned in Section~\ref{}\Bram{Todo}, we need to keep the replay buffer's size limited in order to keep retraining time manageable and to avoid old data from harming the model~\cite{olewicki2022towards}. %However, over time we still want to keep the size of that replay buffer relatively small, so that it does not overpower the training set at each step. 
%Also, previous works observed that old data sometimes harms the model and that ignoring old data can be beneficial~\cite{olewicki2022towards}. %\Do{find the second ref here}
Hence, to ignore older data points, we use a First-In-First-Out (FIFO) approach with the window size $RBWin$ (Replay Buffer Window) as hyperparameter.%a window size of how many samples we want to keep. The size of the window $RBWin$ (for Replay Buffer Window) is a hyper-parameter of the model as well.

\subsubsection{Time step 1: Initialization}

The Lifelong learning set-up has two different types of time steps: first the initialization step, followed by multiple update time steps. 

During the initialization step, the MLP is created and trained for the first time. To do this, we select an initial training window of size $ITWin$ groups. Then, the trained model is used to predict the dependent variable for each data point in the next group ($ITWin+1$) on the timeline. In reality, the test set is not available at training time, but represents actual production data.
During the initialization step, we can define the different sets as: \Bram{double check that the start counts from 1 instead of 0 + "d" for data points}
	\begin{itemize}
		\item Replay buffer: empty
		\item Training set: 
		\{ data points $d$ in group $i$ | $i\in [1; ITWin]$ AND $d  \notin validation$ \} ;
		\item Validation set: 
		\{ data points $d$ in group $i$ | $i\in]ITWin - VWin; ITWin]$ AND $d  \notin training$ \};
		\item Test set: \{ data points $d$ in group $i$ | $i=ITWin$ \}
	\end{itemize}
	%The training and validation set are randomly separated.
	When training the initial MLP model, we used 50 epochs, since our case studies showed that this was enough to pass the under-training stage and to reach the over-training phase. Basically, all 50 epochs are run and the best epoch (in terms of performance on the validation set) is kept as the output of model training, ready for production. 
	At the end of the training, a random sampling is applied to the training set and added to the replay buffer. 
	These samples are balanced to have as many brown as safe build jobs in the replay buffer in the case of brown build detection and risky/non-risky code changes for JIT risk prediction.
	
\subsubsection{Subsequent time steps: Update}
	Once the initial model has been deployed, the strength of LL starts to show upon subsequent time steps, when the MLP model will be updated incrementally. At a given time step $t$, %LL retraining, % for each group on the dataset timeline, at time $t$, the MLP model will be updated.
	the model from $t-1$ is updated with the new data of time group $t$ that has become available, as well as the replay buffer's current state, containing past samples from before $t$. During the time step $t$, we can define the different sets as:
	\begin{itemize}
		\item New data set: \{ data points $d$ in group $i$ | $i=t$ AND $d \notin validation$ \};
		\item Replay buffer: \{ data points $d$ sampled from $i$  | $i\in[t - RBWin; t[$ \};
		\item Training set: New data set $\cup$ Replay buffer;
		\item Validation set: \{ data points $d$ in group $i$ | $i\in]t - VWin; t]$ AND $d \notin training$\} ;
		\item Test set: \{data points $d$ in group $i$ | $i=t+1$\}.
	\end{itemize}
    Again, the test set is not available at the time of retraining, but represents data encountered after deployment in production. %training and validation set or randomly separated for overlapping groups.
    Furthermore, at the end of the training phase, a balanced sampling is done on data group $t$ and added to the replay buffer.
	
\subsection{Empirical study}

The metrics used to evaluate the performance of the approaches for both use cases are F1-score ($F1=\frac{2}{Pre^{-1} + Rec^{-1}}$, where the precision is $Pre=\frac{TP}{TP + FP}$ and recall is $Rec=\frac{TP}{TP + FN}$). The F1-score is the harmonic mean of the precision and recall. We chose to use this metric because of the unbalanced nature of our datasets in terms of $\beta$ and $RR$ in Tables~\ref{} and~\ref{}\Bram{todo}.

As baseline retraining setups to compare LL to, we use the 8 setups of Table~\ref{tab:trainingsetup}. For both use cases, there is a naive AlwaysBrown/Risky baseline corresponding to always predicting builds to be brown, or commits to be risky. For brown build analysis, we also include 2 RFS baselines proposed by Olewicki et al.~\cite{olewicki2022towards}, respectively retraining from scratch each week (Weekly XGB) or based on model performance decay (Heuri XGB). Similarly, for risk prediction, our industry partner provided the actual\Bram{or the authors of Mathieu's paper? (double-blind)} prediction data of an XGBoost model retrained from scratch, using the full data history, at varying points in time (Real pred). Finally, for both use cases, we include baseline retraining setups for MLP models using RFS (RFS NN), and LL models without replay buffer (LL noRB). LL is our own training setup.


% \subsection{Baselines}

% Baselines are explained in Table~\ref{tab:baseline}.

% The brown build detection LL approach will be compared with the state-of-the-art method based on an XGBoost model\cite{olewicki2022towards}, regarding the results of a training-from-scratch approach (every week or after performance decay). 
% XGBoost models are boosted random forest models. Such model, once trained, cannot be updated since trees need to be recomputed entirely, which implies the need of a retraining of the model from scratch when it needs to be updated.
% % The paper thus proposes both a cross-validation and an online validation approach. The former proposes a data splitting into random subsets. The latter retrains the model from scratch each week or after the performance passes under a threshold. 
% The retraining is done using a training window, meaning that the approach already discards old data points.

% Regarding the just-in-time risk prediction use case, we will compare the LL setup with the actual predictions that were done internally by our industrial partner using an XGBoost-based model. The models used for prediction were trained from scratch with all the data available up to the retraining point every few months, but for which we do not have the exact dates.

\begin{table*}[t]
    \centering
    \caption{Training setup baselines.}
    \label{tab:trainingsetup}
    \begin{tabular}{|c|c|p{13cm}|}
    \hline
         Training setup &Use case& Description  \\
         \hline
         AlwaysBrown&Brown& Intuitive baseline where all builds are predicted to be brown \cite{olewicki2022towards}.\\
         AlwaysRisky&Risk& Intuitive baseline where all commits are predicted to be risky.\\
         Weekly XGB&Brown& RFS XGBoost model with training window retrained every week~\cite{olewicki2022towards}.\\
         Heuri XGB&Brown&RFS XGBoost model with a training schedule based on performance decay \cite{olewicki2022towards}.\\
         Real pred&Risk&Industrial collaborator-provided predictions of a RFS XGBoost model with all the available data (unknown schedule) \cite{nayrolles2018clever}.\\
         RFS NN&Brown \& Risk&RFS MLP with all the available data on a group-based schedule.\\
         LL noRB&Brown \& Risk& LL setup with an MLP, retrained on a group-based schedule without replay buffer.\\
         LL&Brown \& Risk&LL setup with an MLP, retrained on a group-based schedule with replay buffer.\\
         \hline
    \end{tabular}
\end{table*}

% \begin{table}[t]
%     \centering
%     \caption{Baseline description}
%     \label{tab:my_label}
%     \begin{tabular}{|c|c|p{4.5cm}|}
%     \hline
%          Name &Use case& Description  \\
%          \hline
%          AlwaysBrown&B& Intuitive baseline where all builds are predicted to be brown.\\
%          Weekly XGB&B& Retrained-from-scratch XGBoost-based model on a weekly schedule.\\
%          Heuri XGB&B&Retrained-from-scratch XGBoost-based model on a heuristic scheduling based on performance decay.\\
%          Real pred&R&Industrial collaborator-provided predictions of a retrained-from-scratch XGBoost-based model (unknown schedule).\\
%          Scratch NN&B \& R&Retrained-from-scratch MLP model on a group-based schedule.\\
%          LL noRB&B \& R& LL setup training of MLP model on a group-based schedule without replay buffer.\\
%          LL&B \& R& LL setup training of MLP model on a group-based schedule with replay buffer.\\
%          \hline
%     \end{tabular}
% \end{table}

==> content/old_files/results.tex <==







\section{RQ1: \RQone}

\paragraph{Motivation}



Using an LL setup allows to update a model more often, and thus to keep the model up-to-date with the newest data acquired, possibly reducing the impact of concept drift. %However, an LL setup sees lower amounts of data at each training step and is at risk for catastrophic forgetting, where previously acquired knowledge gets overwritten. 
In this question, we empirically compare the performance of the LL setup with RFS approaches previously used by our industrial partner. 



\paragraph{Approach}

% Table~\ref{CL_hyper_res} compares LL with the RFS setups baselines. 
For the LL setup, we used the hyperparameter values in Table~\ref{hyper_val}, obtained through a tuning process where each combination of hyperparameters was run 4 times. Table~\ref{CL_hyper_res}, row ``LL'', shows the best average F1-score (over the 4 runs) of the LL retraining setup on the validation set, which we will compare with the RFS setup baselines (Weekly XGB, Heuri XGB and Real Pred).
%Table~\ref{CL_hyper_res} presents the performances of each setup. 
To assess the significance of the performance differences, we use, for each project, a Kruskal-Wallis statistical test to compare the F1-score of the different runs of the LL setup with the other setups.
% The table shows also statistical tests regarding F1-score, the which metric we are optimizing.
% Each line shows the results of the test with ``+'' for a significant difference with large effect size (we did not observe other effect sizes), or ``/'' for a non-significant difference.

\paragraph{Results}
\textbf{The LL setup has an F1-score significantly higher (with large effect) than an RFS setup in 6 projects (from +9\% to +31\%), while performance is similar in the 2 other projects %, the two setups do not show significant performance differences 
(+0\% to +4\%).}

For brown build prediction, when comparing the LL performance with the weekly retraining of an XGBoost model (``Weekly XGB" in Table~\ref{CL_hyper_res}), the F1-score of the LL setup is significantly higher for all projects but Brown\_2. For Brown\_1, the F1-score is 72\% (+16\%), for Brown\_3 31\% (+9\%), and for Brown\_OSS 75\% (+31\%), while for Brown\_2 the F1-score of 71\% still shows a small +4\% increase. %Furthermore, the improvement is significant in all cases, except Brown\_2.
In the case of Brown\_1 and Brown\_OSS, we can see an increase of both the precision (+5\% and +16\%) and recall (+29\% and +55\%).
Brown\_2 and Brown\_3 show a decrease in precision (-7\% and -23\%), which was compensated by an improvement of the recall (+13\% and +32\%), hence an overall improvement of the F1-score as well. The comparison to heuristics-based retraining (row ``Heuri XGB" line in Table~\ref{CL_hyper_res}) is very similar, again with statistical improvements for all projects but Brown\_2.

For JIT risk prediction, we compare the LL setup with our industrial partner's historical model performance (``Real Pred'' in Table~\ref{CL_hyper_res}). 
The F1-score of the LL setup is significantly higher with large effect size for all projects but Risk\_3. For Risk\_1, the F1-score is 56\% (+31\%), for Risk\_2 56\% (+21\%) and for Risk\_4 52\% (+10\%), while for Risk\_3 LL performs identically as Real Pred.
While Risk\_1 and Risk\_2 show a decrease in precision (-24\% and -19\%) compensated by an increase in recall (+47\% and +43\%), Risk\_3 and Risk\_4 show the opposite, with an improvement in precision (+2\% and +15\%) and a reduction in recall (-7\% and -8\%).

We can see that overall, the observations with G-mean are the same as those of the F1-score for all the projects but two, with Risk\_3's real prediction performing significantly better than the LL setup and Risk\_4's real prediction behaving similarly. Note that we tuned the hyper-parameters based on the F1-score, which might explain these observations.


\noindent\doublebox{%
    \parbox{.46\textwidth}{%
        \textbf{RQ1: The LL setup performs at least similarly to the baselines for all datasets and better in 6/8 of the cases.}
    }%
}

\begin{table}[t]
	\centering
	\caption{Optimal hyperparameter values for the LL setup considered in our study.}
	\label{hyper_val}
	\begin{tabular}{|p{2.5cm}|p{.3cm}|p{.3cm}|p{.3cm}|p{.4cm}|p{.3cm}|p{.3cm}|p{.4cm}|p{.3cm}|}
		\hline \multirow{3}{*}{Name}& \multicolumn{8}{c|}{Project's tuned hyperparameters' values}\\\cline{2-9}
	    &\multicolumn{4}{c|}{Brown\_}&\multicolumn{4}{c|}{Risk\_}\\
		\cline{2-9}
		&1&2&3&OSS&1&2&3&4\\\hline

		Group size $GS$&50	&50	&50	&100
		&500&500&1000&500\\
		Initial train window $ITW$&15	&10	&10	&10
		&15&15&15&15\\
		Validation window $VWin$&15		&10		&10		&10
		&8&15&8&8\\
		Replay Buffer sample size [\%$GS$] $RBSize$	&10	&5	&5	&20
		&10&10&10&10\\
		Replay buffer window $RBWin$	&8	&10	&5	&10
		&8&15&8&8\\
		\hline
	\end{tabular}
\end{table}

\section{RQ2: \RQonebis}

\paragraph{Motivation}

While in RQ1 we observe favorable performance of the LL approach compared to the RFS baselines, the question still remains to what extent these performance improvements are related to the choice for LL or the choice for using a NN-based model. Hence, here we compare an NN-based RFS approach to the NN-based LL approach.



\paragraph{Approach}

The RFS MLP baseline uses the same MLP model and scheduling approach as the LL setup, as mentioned in Table~\ref{tab:trainingsetup} (RFS MLP).
We compare it with the LL setup from the previous section, using the same Kruskal-Wallis test. Results are shown in Table~\ref{CL_hyper_res}.

\paragraph{Results}

\textbf{Out of the 8 datasets, 3 show a significant improvement in F1-score (+5-8\%) for the LL setup compared to an RFS MLP, 4 show no significant difference (-1\% to +8\%), and 1 shows a significant decrease (-5\%).}

In Table~\ref{CL_hyper_res}, we observe that using an LL setup significantly improves the F1-score in comparison to RFS MLP for Brown\_1 (+8\%), 
%Brown\_2 (+1\%), 
Brown\_OSS (+5\%), and
%Risk\_2 (+8\%) and 
Risk\_4 (+5\%). In contrast, %, among which Brown\_2 and Risk\_2 are not significant improvements. 
Brown\_3 
%and Risk\_2 
shows a significant decrease in F1-score (-5\% significant% and -1\% non-significant
). In the other cases, LL performed at least as well as RFS MLP.
Regarding the G-mean, the same observations can be made apart from Brown\_1 not having a significant improvement, still achieving a +8\% increase. 

In terms of precision and recall, no clear patterns could be discerned neither by dataset nor by training setup. For the case of Brown\_3 (where LL performed significantly less with large effect size), we noticed a decrease in precision (-5\%) and recall (-4\%) for the LL setup. This shows that in this case, seeing all of the past data actually improved the performance, which we suspect is due to the very unbalanced dataset ($\beta$ of 5\%), causing LL to overtrain on the few brown jobs, while RFS has access to all historical jobs.
Two of the four projects with equal performance have a heavily cyclic development process of 3-month sprints; future empirical analysis should investigate the potential link between these process characteristics and the model results.



\noindent\doublebox{%
    \parbox{.46\textwidth}{%
        \textbf{RQ2: The LL setup performs similarly to RFS setups in 4/8 cases, outperforms them in 3/8 datasets, and is outperformed in 1 case. Hence, LL can bring value in terms of model performance, but is not a panacea.}
    }%
}


% \begin{table*}[t]
%     \centering
%     \caption{Performance after hyper-parameter optimization for the LL models and baselines. The \textcolor{cyan}{\textbf{bold blue}} values indicate the best F1-score per project.
%     For each project, Kruskal-Wallis tests ($\alpha=.05$) between the F1-score of \conditional{runs of} the LL setup and of the other setups are performed. If significant, the Cliff's delta effect size is shown as ``+'' (large effect), otherwise ``/'' is shown.}
%     \label{CL_hyper_res}
%     \begin{tabular}{|p{1.7cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}|}
%     	\hline
%     	\multirow{3}{*}{Model}& \multicolumn{5}{c|}{Project Brown\_1} 
%     	& \multicolumn{5}{c|}{Project Brown\_2}& \multicolumn{5}{c|}{Project Brown\_3} 
%     	& \multicolumn{5}{c|}{Project Brown\_OSS} \\ \cline{2-21}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}\\
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}\\ 
%     	\hline
%         Weekly XGB&56 +&59&54&84&81
%     	&67 /&75&61&88&79
%     	&22 + &45&15&99&95
%     	&44 +&44&45&98&98\\
%     	Heuri XGB&60 +&61&60&84&83
%     	&67 /&73&62&86&79
%     	&27 +&50&19&99&96
%     	&44 +&44&45&98&98\\
%     	RFS MLP&
%     	64 + & 53&80&84&59&
%     	70 /&68&72&73&69&
%     	\textcolor{cyan}{\textbf{36}} +&28&51&89&75&
%     	70 +&68&72&73&69\\
%     	LL noRB
%     	&66 /&54&83&85&58
%         &68 /&64&74&71&61	
%         &30 /&21&52&87&63
%     	&49 +&33&100&100&65  \\
% 		LL&\textcolor{cyan}{\textbf{72}} &{64}&{83}&{88}&{72}%&3min23
% 	&\textcolor{cyan}{\textbf{71}} &{68}&{74}&{74}&{68}
% 	    & 31 &{23}&{47}&{87}&{69}%&5min15
%     	&\textcolor{cyan}{\textbf{75}} &{60}&{100}&{100}&{89}\\
    	
%     	\hline
%     	\hline
%     	\multirow{3}{*}{Model}& \multicolumn{5}{c|}{Project Brown\_1} 
%     	& \multicolumn{5}{c|}{Project Brown\_2}& \multicolumn{5}{c|}{Project Brown\_3} 
%     	& \multicolumn{5}{c|}{Project Brown\_OSS} \\ \cline{2-21}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}
%     	&\multicolumn{3}{p{.6cm}|}{Brown}&\multicolumn{2}{p{.4cm}|}{Safe}\\
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}\\ 
%     	\hline
%     	Real Pred
%     	&25 +&74&15&78&98
%         &35 +&66&24&77&95
%         &59 /&45&88&95&66
%         &42 +&29&74&94&69\\
%         RFS MLP&
%         \textcolor{cyan}{\textbf{57}} /&51&65&85&76&
%         48 /&36&74&77&40&
%         59 /&47&78&85&58&
%         47 +&38&61&87&72\\
%         LL noRB 
%         &52 + &44&64&84&69
%         &50 /&40&67&79&62
%         &\textcolor{cyan}{\textbf{60}} /&50&75&84&64
%         &45 +&34&69&88&64\\
%         LL
%         &56 &50&62&84&76
%         &\textcolor{cyan}{\textbf{56}} &47&67&82&66
%         &59 &47&81&86&58
%         &\textcolor{cyan}{\textbf{52}} &44&66&89&75\\
%         \hline
%     \end{tabular}
% \end{table*}


% \begin{table*}[t]
%     \centering
%     \caption{Performance after hyper-parameter optimization for the LL models and baselines. The \textcolor{cyan}{\textbf{bold blue}} values indicate the best F1-score (F1) and G-mean (GM) per project.
%     For each project, Kruskal-Wallis tests ($\alpha=.05$) between the F1-score/G-mean of \conditional{runs of} the LL setup and of the other setups are performed. If significant, the Cliff's delta effect size is shown as ``+'' (large effect), otherwise ``/'' is shown.}
%     \label{CL_hyper_res}
%     \begin{tabular}{|p{1.7cm}|
%                 lp{.2cm}p{.2cm}p{.4cm}l|
%                 lp{.2cm}p{.2cm}p{.4cm}l|
%                 lp{.2cm}p{.2cm}p{.4cm}l|
%                 lp{.2cm}p{.2cm}p{.4cm}l|}
%     	\hline
%     	\multirow{3}{*}{Model}
%             & \multicolumn{5}{c|}{Project Brown\_1} 
%     	& \multicolumn{5}{c|}{Project Brown\_2}
%             & \multicolumn{5}{c|}{Project Brown\_3} 
%     	& \multicolumn{5}{c|}{Project Brown\_OSS} \\ \cline{2-21}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}\\
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&\\ 
%     	\hline
%         Weekly XGB&56 +&59&54&81&66 +
%     	&67 /&75&61&79&69 +
%     	&22 + &45&15&95&37 +
%     	&44 +&44&45&98&66 +\\
%     	Heuri XGB&60 +&61&60&83&71 +
%     	&67 /&73&62&79&70 +
%     	&27 +&50&19&96&43 +
%     	&44 +&44&45&98&66 +\\
%     	RFS MLP&
%     	64 + & 53&80&59&69 /&
%     	70 /&68&72&69&70 /&
%     	\textcolor{cyan}{\textbf{36}} +&28&51&75&\textcolor{cyan}{\textbf{62}} +&
%     	70 +&68&72&69&70 +\\
%     	LL noRB
%     	&66 /&54&83&58&69 /
%         &68 /&64&74&61	&67 /
%         &30 /&21&52&63&57 /
%     	&49 +&33&100&65 & 81 +\\
% 		LL&\textcolor{cyan}{\textbf{72}} &{64}&{83}&{72}&\textcolor{cyan}{\textbf{77}}%&3min23
% 	&\textcolor{cyan}{\textbf{71}} &{68}&{74}&{68}&\textcolor{cyan}{\textbf{71}}
% 	    & 31 &{23}&{47}&{69}&57%&5min15
%     	&\textcolor{cyan}{\textbf{75}} &{60}&{100}&{89}&\textcolor{cyan}{\textbf{94}}\\
    	
%     	\hline
%     	\hline
%     	& \multicolumn{5}{c|}{Project Risk\_1} 
%     	& \multicolumn{5}{c|}{Project Risk\_2}
%             & \multicolumn{5}{c|}{Project Risk\_3} 
%     	& \multicolumn{5}{c|}{Project Risk\_4} \\ \cline{2-21}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{1}{p{.2cm}|}{Safe}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}\\
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}&\\ 
%     	\hline
%     	Real Pred
%     	&25 +&74&15&98&38 +
%         &35 +&66&24&95&48 /
%         &59 /&45&88&66&76 +
%         &42 +&29&74&69&\textcolor{cyan}{\textbf{71}} /\\
%         RFS MLP&
%         \textcolor{cyan}{\textbf{57}} /&51&65&76&\textcolor{cyan}{\textbf{70}} /&
%         48 /&36&74&40&54 /&
%         59 /&47&78&58&67 /&
%         47 +&38&61&72&66 +\\
%         LL noRB 
%         &52 + &44&64&69&66 +
%         &50 /&40&67&62&64 /
%         &\textcolor{cyan}{\textbf{60}} /&50&75&64&\textcolor{cyan}{\textbf{69}} /
%         &45 +&34&69&64&66 +\\
%         LL
%         &56 &50&62&76&69
%         &\textcolor{cyan}{\textbf{56}} &47&67&66&\textcolor{cyan}{\textbf{66}}
%         &59 &47&81&58&68
%         &\textcolor{cyan}{\textbf{52}} &44&66&75&70\\
%         \hline
%     \end{tabular}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{Performance after hyper-parameter optimization for the LL models and baselines. The \textcolor{cyan}{\textbf{bold blue}} values indicate the best F1-score (F1) and G-mean (GM) per project.
    For each project, Kruskal-Wallis tests ($\alpha=.05$) between the F1-score/G-mean of runs of the LL setup and of the other setups are performed. If significant, the Cliff's delta effect size is shown as ``+'' (large effect), otherwise ``/'' is shown.}
    \label{CL_hyper_res}
    \begin{tabular}{|p{1.6cm}|
                llp{.2cm}p{.2cm}p{.4cm}|
                llp{.2cm}p{.2cm}p{.4cm}|
                llp{.2cm}p{.2cm}p{.4cm}|
                llp{.2cm}p{.2cm}p{.4cm}|}
    	\hline
    	\multirow{3}{*}{Model}
            & \multicolumn{5}{c|}{Project Brown\_1} 
    	& \multicolumn{5}{c|}{Project Brown\_2}
            & \multicolumn{5}{c|}{Project Brown\_3} 
    	& \multicolumn{5}{c|}{Project Brown\_OSS} \\ \cline{2-21}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	\\
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}\\ 
    	\hline
        Weekly XGB&56 +&66 +&59&54&81
    	&67 /&69 +&75&61&79
    	&22 + &37 +&45&15&95
    	&44 +&66 +&44&45&98\\
    	Heuri XGB&60 +&71 +&61&60&83
    	&67 /&70 +&73&62&79
    	&27 +&43 +&50&19&96
    	&44 +&66 +&44&45&98\\
    	RFS MLP&
    	64 + & 69 /&53&80&59&
    	70 /&70 /&68&72&69&
    	\textcolor{cyan}{\textbf{36}} +&\textcolor{cyan}{\textbf{62}} +&28&51&75&
    	70 +&70 +&68&72&69\\
    	LL noRB
    	&66 /&69 /&54&83&58
        &68 /&67 /&64&74&61	
        &30 /&57 /&21&52&63
    	&49 +& 81 +&33&100&65 \\
		LL&\textcolor{cyan}{\textbf{72}}&\textcolor{cyan}{\textbf{77}} &{64}&{83}&{72}%&3min23
	&\textcolor{cyan}{\textbf{71}}&\textcolor{cyan}{\textbf{71}} &{68}&{74}&{68}
	    & 31 &57&{23}&{47}&{69}%&5min15
    	&\textcolor{cyan}{\textbf{75}}&\textcolor{cyan}{\textbf{94}} &{60}&{100}&{89}\\
    	
    	\hline
    	\hline
            \multirow{3}{*}{Model}
    	& \multicolumn{5}{c|}{Project Risk\_1} 
    	& \multicolumn{5}{c|}{Project Risk\_2}
            & \multicolumn{5}{c|}{Project Risk\_3} 
    	& \multicolumn{5}{c|}{Project Risk\_4} \\ \cline{2-21}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}
     &\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}
     &\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}
     &\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}\\
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}\\ 
    	\hline
    	Real Pred
    	&25 +&38 +&74&15&98
        &35 +&48 /&66&24&95
        &59 /&\textcolor{cyan}{\textbf{76}} +&45&88&66
        &42 +&\textcolor{cyan}{\textbf{71}} /&29&74&69\\
        RFS MLP&
        \textcolor{cyan}{\textbf{57}} /&\textcolor{cyan}{\textbf{70}} /&51&65&76&
        48 /&54 /&36&74&40&
        59 /&67 /&47&78&58&
        47 +&66 +&38&61&72\\
        LL noRB 
        &52 + &66 +&44&64&69
        &50 /&64 /&40&67&62
        &\textcolor{cyan}{\textbf{60}} /&69 /&50&75&64
        &45 +&66 +&34&69&64\\
        LL
        &56&69 &50&62&76
        &\textcolor{cyan}{\textbf{56}}&\textcolor{cyan}{\textbf{66}} &47&67&66
        &59&68 &47&81&58
        &\textcolor{cyan}{\textbf{52}} &70&44&66&75\\
        \hline
    \end{tabular}
\end{table*}


% \begin{table*}[t]
%     \centering
%     \caption{Performance after hyper-parameter optimization for the LL models and baselines. The \textcolor{cyan}{\textbf{bold blue}} values indicate the best F1-score (F1) and G-mean (GM) per project.
%     For each project, Kruskal-Wallis tests ($\alpha=.05$) between the F1-score of \conditional{runs of} the LL setup and of the other setups are performed. If significant, the Cliff's delta effect size is shown as ``+'' (large effect), otherwise ``/'' is shown.}
%     \label{CL_hyper_res}
%     \begin{tabular}{|p{1.7cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}p{.2cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}p{.2cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}p{.2cm}|
%                 lp{.2cm}p{.2cm}p{.2cm}p{.2cm}p{.2cm}|}
%     	\hline
%     	\multirow{3}{*}{Model}
%             & \multicolumn{6}{c|}{Project Brown\_1} 
%     	& \multicolumn{6}{c|}{Project Brown\_2}
%             & \multicolumn{6}{c|}{Project Brown\_3} 
%     	& \multicolumn{6}{c|}{Project Brown\_OSS} \\ \cline{2-21}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}&\multicolumn{1}{p{.2cm}|}{G}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}&\multicolumn{1}{p{.2cm}|}{G}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}&\multicolumn{1}{p{.2cm}|}{G}
%     	&\multicolumn{3}{c|}{Brown}&\multicolumn{2}{c|}{Safe}&\multicolumn{1}{p{.2cm}|}{G}\\
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{M}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{M}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{M}
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{M}\\ 
%     	\hline
%         Weekly XGB&56 +&59&54&84&81&66
%     	&67 /&75&61&88&79&69
%     	&22 + &45&15&99&95&37
%     	&44 +&44&45&98&98&66\\
%     	Heuri XGB&60 +&61&60&84&83&71
%     	&67 /&73&62&86&79&70
%     	&27 +&50&19&99&96&43
%     	&44 +&44&45&98&98&66\\
%     	RFS MLP&
%     	64 + & 53&80&84&59&69&
%     	70 /&68&72&73&69&70&
%     	\textcolor{cyan}{\textbf{36}} +&28&51&89&75&\textcolor{cyan}{\textbf{62}}&
%     	70 +&68&72&73&69&70\\
%     	LL noRB
%     	&66 /&54&83&85&58&69
%         &68 /&64&74&71&61	&67
%         &30 /&21&52&87&63&57
%     	&49 +&33&100&100&65 & 81\\
% 		LL&\textcolor{cyan}{\textbf{72}} &{64}&{83}&{88}&{72}&\textcolor{cyan}{\textbf{77}}%&3min23
% 	&\textcolor{cyan}{\textbf{71}} &{68}&{74}&{74}&{68}&\textcolor{cyan}{\textbf{71}}
% 	    & 31 &{23}&{47}&{87}&{69}&57%&5min15
%     	&\textcolor{cyan}{\textbf{75}} &{60}&{100}&{100}&{89}&\textcolor{cyan}{\textbf{94}}\\
    	
%     	\hline
%     	\hline
%     	& \multicolumn{6}{c|}{Project Risk\_1} 
%     	& \multicolumn{6}{c|}{Project Risk\_2}
%             & \multicolumn{6}{c|}{Project Risk\_3} 
%     	& \multicolumn{6}{c|}{Project Risk\_4} \\ \cline{2-21}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{2}{p{.4cm}|}{Safe}&\multicolumn{1}{c|}{\multirow{2}{*}{G}}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{2}{p{.4cm}|}{Safe}&\multicolumn{1}{c|}{\multirow{2}{*}{G}}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{2}{p{.4cm}|}{Safe}&\multicolumn{1}{c|}{\multirow{2}{*}{G}}
%     	&\multicolumn{3}{c|}{Risk}&\multicolumn{2}{p{.4cm}|}{Safe}&\multicolumn{1}{c|}{\multirow{2}{*}{G}}\\
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&
%     	&F1&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\\ 
%     	\hline
%     	Real Pred
%     	&25 +&74&15&78&98&38
%         &35 +&66&24&77&95&48
%         &59 /&45&88&95&66&76
%         &42 +&29&74&94&69&\textcolor{cyan}{\textbf{71}}\\
%         RFS MLP&
%         \textcolor{cyan}{\textbf{57}} /&51&65&85&76&\textcolor{cyan}{\textbf{70}}&
%         48 /&36&74&77&40&54&
%         59 /&47&78&85&58&67&
%         47 +&38&61&87&72&66\\
%         LL noRB 
%         &52 + &44&64&84&69&66
%         &50 /&40&67&79&62&64
%         &\textcolor{cyan}{\textbf{60}} /&50&75&84&64&\textcolor{cyan}{\textbf{69}}
%         &45 +&34&69&88&64&66\\
%         LL
%         &56 &50&62&84&76&69
%         &\textcolor{cyan}{\textbf{56}} &47&67&82&66&\textcolor{cyan}{\textbf{66}}
%         &59 &47&81&86&58&68
%         &\textcolor{cyan}{\textbf{52}} &44&66&89&75&70\\
%         \hline
%     \end{tabular}
% \end{table*}


\section{RQ3: \RQtwo}
\paragraph{Motivation}

 LL setups are often at risk of showing symptoms of catastrophic forgetting, gradually decreasing the performance of LL retraining. To reduce this risk, we adopt a replay buffer (memory-based approach). In this question, we aim at evaluating how impactful this approach is on LL.

\paragraph{Approach}

We compare the LL setup with(out) replay buffer, corresponding respectively to rows ``LL"/``LL noRB" in Table~\ref{CL_hyper_res}.

\paragraph{Results}

\textbf{Using a replay buffer significantly improved the F1-score for 3 projects (from +4\% to +26\%) and did not significantly change the performance for the other 5 projects (from -1\% to +6\%).}

%In Table~\ref{CL_hyper_res}, the "LL noRB" lines show performance of an LL setup without replay buffer for all the studied datasets. 
In Table~\ref{CL_hyper_res}, we observe that using a replay buffer statistically significantly improves the F1-score (with large effect size) for Brown\_OSS (+26\%), Risk\_1 (+4\%), and Risk\_4 (+7\%). While Risk\_3 sees an F1-score decrease by 1\%, the difference in performance is not significant. Brown\_OSS sees an improvement in precision (from +3\% to +27\%), without any change in recall, while Risk\_1 and Risk\_4 have a lower recall (-2\% and -3\%) that is compensated by an increase in precision (+6\% and +10\%). 
The G-mean observations are similar to those of the F1-score.



\noindent\doublebox{%
    \parbox{.46\textwidth}{%
        \textbf{RQ3: The use of a memory-based approach (replay buffer) to reduce catastrophic forgetting significantly improves the performance for 3 out of 8 projects, while maintaining performance for the others.}
    }%
}


\begin{table}[t]
    \centering
    \caption{Average Life Expectation of models in \#days.}
    \label{time_group}
    \begin{tabular}{|l|c|c|c|c|}
    	\hline
    	Life Exp [day]&Brown\_1&Brown\_2&Brown\_3&Brown\_OSS\\ \hline
    	Weekly XGB & 7&7&7&7\\
    	Heuri XGB&42&35&14&7\\
    	LL (med.)&9&4&5&18\\
    	LL (avg.)&12$\pm$3&12$\pm$9&6$\pm$2&85$\pm$99\\
    	\hline
    	\hline
    	Life Exp [day]&Risk\_1&Risk\_2&Risk\_3&Risk\_4\\ \hline
    	Real Pred &$49\pm$7&$49\pm$7&$49\pm$7&$49\pm$7\\ 
    	LL (med.)&32&22&35&36\\ 
    	LL (avg.)&40$\pm$11&32$\pm$6&43$\pm$6&32$\pm$13\\ 
        \hline
    \end{tabular}
\end{table}

\begin{table}[t]
    \centering
    \caption{Size of training sets for model training/updates in terms of $GS$ for all datasets, and average model computation time across 5 runs for the Risk datasets (training with 50 epochs and 10 sample batches).}
    \label{datasets_size}
    \begin{tabular}{|l|c|c|c|c|}
    	\hline
    Dataset size &Brown\_1&Brown\_2&Brown\_3&Brown\_OSS\\ \hline
    	RFS XGB (med)& 24.6$GS$&11.4$GS$&10.5$GS$&6.6$GS$\\
    	LL initializat.&15$GS$&10$GS$&10$GS$&10$GS$\\
    	LL updates&1.8$GS$&1.5$GS$&1.25$GS$&2$GS$\\
        LL Speedup&8.3&6.7&8.&5.\\
    	\hline
    	\hline
    	Dataset size &Risk\_1&Risk\_2&Risk\_3&Risk\_OSS\\ \hline
    	LL initializat.&15$GS$&15$GS$&15$GS$&15$GS$\\
    	LL updates&1.8$GS$&2.5$GS$&1.8$GS$&1.8$GS$\\ 
        LL Speedup&8.3&6.&8.3&8.3\\
            \hline
        Avg. time [s] &Risk\_1&Risk\_2&Risk\_3&Risk\_OSS\\ 
     \hline
        LL initializat.&38.6&121.4&91.9&32.7\\
        LL updates&10.4&12.7&11.4&9.\\ 
        LL Speedup&3.7&9.6&8.1&3.6\\
        \hline
    \end{tabular}
\end{table}


\section{RQ4: \RQthree}
\paragraph{Motivation}

From RQ1, we observe that the LL setup performs at least as well as state-of-the-art RFS approaches for cases. RQ2 shows that it is not a panacea, still performing at least as good than an MLP RFS setup in 7/8 cases. RQ2 highlights that it is not a panacea, still performing  However, since model retraining is now performed more frequently, the combined computational effort across all model retraining attempts might outweigh the single model retraining computation of RFS. 
This might make LL less tempting to adopt, especially in the cases where LL did not outperform the RFS models.
Hence, %Besides evaluating the performance of both setups, we want to compare their computation efforts. 
in this RQ, we evaluate how often updates are necessary as well as approximations of the actual computational effort of update/model training.


\paragraph{Approach}

We model the overall computational effort for both retraining setups in terms of the life expectation of models and the complexity of the retraining algorithms~\cite{wilf2002algorithms}. First, the life expectation (LifeExp) of a model corresponds to the time between successive model updates.
For each project and a given retraining setup, Table~\ref{time_group} shows the median life expectation across all retraining attempts. 

Secondly, as done by Thuijsman et al.~\cite{thuijsman2019computational}, we calculate the algorithms' complexity in terms of the size of the training set $TrainS$.
As shown in Algorithm~\ref{algo_nn}, the update/training time of our MLP models is linearly dependent on the size of the training set, as is the complexity of XGBoost training algorithm~\cite{chen2016xgboost}. In other words, we can compare the computational effort of RFS and LL retraining setups by comparing the training data sizes. 

To combine both measures into one measure of computational effort for retraining, we define the effort coefficient $coef$=$\frac{trainS}{lifeExp}$ and the relative coefficient $coef_{rel}$=$\frac{coef}{coef[LL]}$, which is relative to the coefficient of the LL setup. The higher the coef\_rel for a given training setup, the more retraining effort it requires compared to LL.


\paragraph{Results}

\textbf{The median life expectation of models with an LL setup is between 1.1-8.75 times shorter than the best baseline for 7 of the studied projects and is 2.3 times longer for Brown\_OSS.}

Table~\ref{time_group} shows how, in the case of brown build prediction, the median life expectation of LL models for Brown\_1, 2 and 3 is 2.8-8.75 times shorter than for Heuri XGB, needing thus more updates for similar to significantly better model performance (cf. RQ1). On the other hand, for Brown\_OSS, the median life expectation of models is 2.3 times longer than for both XGB-based baselines because that project has much slower brown build activity, if we refer to the total age of the project and the amount of brown jobs from Table~\ref{info_proj}. Since less frequent brown jobs are encountered, training more often (with smaller $GS$) would most likely overfit on the lower amount of brown jobs present in the training set.

For JIT risk prediction, the LL model needs updates every .6-1 month as a median in the LL setup, whereas the actual RFS is done every 1.5-2 months by our industrial partner (Real Pred), having thus a median life expectation 1.1-2.2 times shorter with the LL setup.

\textbf{The LL updates use about 3.3-13.7 times less data during updates than the RFS approach.}

Similar to Olewicki et al.~\cite{olewicki2022towards}, we found that the RFS approach for brown build detection requires an optimal training dataset size of 30 weeks for all studied projects. To put this in context, we express this in terms of the median $GS$ (in terms of number of commits) of data groups used by LL in Table~\ref{datasets_size} (row ``RFS XGB (med)"). 
The LL initialization step (which is equivalent to an RFS) uses a training set of $ITW$ time groups (see Table~\ref{hyper_val}), with each group containing $GS$ data points. We consider the resulting $\sim 10$-$15~GS$ data points as a lower bound for the dataset size in an RFS MLP setup.
Later model updates use a training set composed of both new data points that happened since the last update and a replay buffer, amounting to $GS + \frac{RBSSize}{100}\times RBWin \times GS$ data points. 

When comparing in Table~\ref{datasets_size} the training set sizes of the LL updates to RFS XGB for brown build detection (no XGB information was available for JIT), the dataset of LL updates is 3.3-13.7x smaller (\eg $24.6/1.8$=$13.7$ for Brown\_1). Then, when comparing LL updates with LL initialization (row ``LL Speed up''), this time on all 8 projects, we find that the dataset of LL updates is 5-8.3x smaller than the LL initialization. For JIT, the former dataset is 3.6-9.6x smaller.

Figure~\ref{fig:coef_rel} shows that the relative effort coefficient $coef_{rel}$ for all the setups is between 2 and 40, showing the overall lower computational effort of the LL setup.


\textbf{The actual model retraining time speedup matches the theoretical one for 2/4 Risk datasets, and is at least 3.6-fold for the others.}

%As an example, we uploaded the mean computation time for the Risk datasets online~\cite{todo} as well as the ratio of initialisation/update time (measuring speedup of LL compared to RFS in terms of time). In half of the cases, the speedup in terms of time matches the theoretically expected speedup (linear dependency on data file size), while the LL time efficiency is still at least 3.6 times as high for the others, yet limited by the standard Python library we used.
Table~\ref{datasets_size} shows an example of the actual mean computation time for initialization and updates of the MLP model in an LL setup for the Risk datasets. The LL Speedup ratio ($\frac{init}{update}$) is given as a measure to compare LL to RFS computational effort, as RFS takes a similar time as the LL initialization time for each retraining. 
In half of the projects, the speedup in terms of time matches the theoretically expected speedup (linear dependency on data file size), while the LL time efficiency is still at least 3.6x as high for the others, yet limited by the standard Python library used.


% We observe how the actual ratio ranges from 3.6 to 9.6, showing substantial improvements in training time over RFS. In two cases, the actual ratio matches or even exceeds the expected ratio, while in two other cases the actual ratio is about 2.2 times lower than the expected ratio. This happens for a number of reasons such as the over-sampling in the training set depending on the data imbalance of each time step, and certain computations happening at both initialization and update times that are either constant time (e.g., NN's optimizer reset, validation prediction for early stopping) or close to constant time (e.g., batch creation $\sim$ ln(n)). The latter issue's impact could be lowered by using optimized Python libraries for such computations instead of the standard API libraries.
% \begin{table}[t]
% \centering
% \caption{Average computational time for model initianisation and update of NN-models with 50 epochs and 10 sample batches (average on 5runs).}\label{time}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Dataset} & Initialisation & Update& actual & expected\\
%  & time [s] & time [s] & ratio & ratio\\ \hline
% Risk\_1 & 38.6 & 10.4 & 3.7 & 8.3\\
% Risk\_2 & 121.7 & 12.7 & 9.6 & 6\\
% Risk\_3 & 91.9 & 11.4 & 8.1 & 8.3\\
% Risk\_4 & 32.7 & 9.0 & 3.6 & 8.3\\
% \hline
% \end{tabular}
% \end{table}


\noindent\doublebox{%
    \parbox{.46\textwidth}{%
        \textbf{
        RQ4: The computational effort of maintaining an LL setup is 2-40x less expensive than an RFS setup. %Even though the LL setup needs 1.1-8.75x more frequent updates, The actual computational effort for updating the model is 3.3-13.7xlower.
        }
    }%
}
\begin{figure}
     \centering
    \includegraphics[width=.45\textwidth]{img/coef_rel.png}
    \caption{Relative coefficient $coef_{rel}$ of training setups compared to the LL setup updates.}
    \label{fig:coef_rel}
\end{figure}






==> content/old_files/usecases.tex <==



\begin{table*}[h]
	\centering
	\caption{\label{info_proj} Information on the projects studied.}
	
	\vspace{-0.3cm}
	
	\begin{tabular}{|c||p{1.cm}|r|p{1.4cm}|p{.4cm}||r|r|p{1.cm}|p{1.8cm}|p{2cm}|}
		\hline
		\multirow{2}{*}{\textbf{Proj}}&\multicolumn{4}{c||}{\textbf{Full project history}}&\multicolumn{5}{c|}{\textbf{Scraped data}}\\
		\cline{2-10}
		&\textbf{\#Contri- butors}&\textbf{\#commit}&\textbf{Main Languages}&\textbf{Age} [y]&\textbf{\#months}&\textbf{\#jobs}&\textbf{\#failing jobs}&\textbf{Brown failure rate~($\beta$)}&\textbf{Mean job duration }$[$mm:ss$]$\\
		\hline
		Brown\_1&15&3k&Go, JS&3.5 &18&23k&3008&30\%&03:27$\pm$04\\ %Clever 2017-03
		Brown\_2&29&2k&C\#&4                         &29&63k&8100&37\%&03:14$\pm$14\\ %GearStudio 2012-09
		Brown\_3&64&7k&C++, C&3                         &17&22k&5986&5\%&15:49$\pm$30\\%GearCore 2012-01
		Brown\_OSS&20&14k&C,C++&17&43&47k&1237&13\%&06:12$\pm$17\\
		\hline
	\end{tabular}
\end{table*}


\begin{table}[t]
	\centering
	\caption{\label{risk:info_proj} Information on the studied projects for Just-In-Time risk prediction. The Risk rate represent the percentage of risky file in the all dataset.}
	
	\begin{tabular}{|c|c|c|c|c|}%{|c||p{1.cm}|r|p{1.4cm}|p{.4cm}||p{1.2cm}|r|r|p{1.cm}|p{1.8cm}|p{2cm}|}
		\hline
		\multirow{2}{*}{\textbf{Project}}&\textbf{Age}&\textbf{\#commits}&\textbf{\#risky-}&\textbf{Risky rate}\\
		&[y]&&\textbf{commits}&\textbf{($RR$)}\\
		\hline
		Risk\_1&5&50k&12k&24\%\\
		Risk\_2&4&49k&13k&27\%\\
		Risk\_3&9&82k&20k&24\%\\
		Risk\_4&5&57k&9k&15\%\\
		\hline
	\end{tabular}
\end{table}

\begin{table}[t]
	\centering
\caption{\label{risk:info_feat} Features used for Just-In-Time risk prediction.}
	
	\begin{tabular}{|p{2cm}|p{6cm}|}%{|c||p{1.cm}|r|p{1.4cm}|p{.4cm}||p{1.2cm}|r|r|p{1.cm}|p{1.8cm}|p{2cm}|}
		\hline
		\textbf{Name}&\textbf{Description}\\
		\hline
		Subsystems&Number of modified subsystems. A subsystem is directory containing code files.\\
		Files& Number of modified, added or deleted files.\\
		Line added& Number of added lines of code.\\
		Line deleted& Number of deleted lines of code.\\
		Line total& Number of modified lines of code (added and deleted).\\
		Devs& Number of developers who changed the modified files.\\
		Age& Age of the file.\\
		Unique change& Number of unique changes.\\
		Experience& Experience of the developer who submitted the code change. All types of experiences are measured in terms of contributions weighted over-time $1/(m-1)$ where $m$ is the elapsed months since the contribution.  \\
		Reviewers& Number of reviewers assigned to the code change.\\
		Reviewers\_ experiences& Experience of the reviewers in reviewing the modified files. \\
		Reviewers\_ dev\_experiences& Experience of the reviewers in editing the modified files.\\
		Reviewers\_ subsystem\_ experiences& Experience of the reviewers in reviewing the modified subsystems.\\
		Approvers& Number of approvers assigned to the code change.\\
		Approvers\_ experiences& Experience of the approvers in approving changes to the modified files. \\
		Approvers\_ dev\_experiences& Experience of the approvers with the dev. who submitted the code change.\\
		Approvers\_ subsystem\_ experiences& Experience of the approvers in editing the modified files.\\
		FilesRiskiness & Historical rate of bug introducing changes in the modified files.\\
		Subsystems-Riskiness & Historical rate of bug introducing changes in the modified subsystems.\\
% 		Hour&Time of submission\\
% 		Day&Day of submission\\
% 		Month&Month of submission\\
% 		Weekday&Weekday of submission\\
		Daytorelease&Number of days to the release date of next update of the software product.\\
		\hline
	\end{tabular}
\end{table}

Our empirical study involves two software analytics tools used in the CI pipelines of our industrial partner, applied to 7 closed-source and 1 open-source datasets. %provided by our industrial partner, a game development company.
The software analytics tools are used in the context of our industrial partner are being used from 3 to 5 years on a given project. One tool performs brown build detection tool~\cite{olewicki2022towards}, while the other performs JIT risk prediction~\cite{nayrolles2018clever}. The features used in these tools are build traces and metrics related to code changes.
What sets apart software analytics tools for game development from regular software development, is the need for said tools to deal with a multitude of different types of file content, from source code itself, to sound files, or behavioral trees, textures and other assets needed for the game. Furthermore, game development follows a well-defined process of steps/gates, each implying different objectives and hence potentially changing distributions in software engineering data. %thus different ways of developing.

%For now, we consider two use cases, a brown build detection tool~\cite{olewicki2022towards}, and a JIT risk prediction tool~\cite{nayrolles2018clever}. The features used in these tools are build traces and metrics related to code changes.
%Our industrial partner is providing closed-source datasets to work with. We are also considering one open-source dataset from other software development projects. 



\subsection{Brown Build detection}

\subsubsection{Description}

Continuous Integration (CI) evaluates the quality and security of new code changes submitted to the integration pipeline by executing builds and test jobs~\cite{shahin2017continuous}.
In theory, successful builds validate the changes, whereas failed builds indicate the need to rectify the code change before integrating it to the project. In practice, the difference between successful and failed builds is blurred by so-called ``brown builds''.
%CI services such as TravisCI or Jenkins generate build scripts that run compilations and tests on code changes regarding different environments/operating systems that need to be covered by the developed project~\cite{zolfagharinia2017not}. 
%In theory, for each code change, a series of builds need to be triggered. 
%Over time, with the number of features and of environments increasing, the number of triggered builds increases generating a build inflation~\cite{zolfagharinia2019study}.
%To reduce this inflation, several code changes will be dealt with as a group, which reduces the number of builds needed if the group level builds all succeed, but causes additional build job if builds fail. Furthermore, due to the build inflation, the interpretability of build failure at group level can become challenging~\cite{ziftci2017broke}.

%Besides build inflation, the issue of brown builds can also cripple CI pipelines. 
A brown build (or flaky build) is defined as an intermittent build job failure, that would change to success just by rerunning the build~\cite{lampel2021life}.
Those inconsistent build failures are often attributed to the build scripts itself~\cite{ghaleb2019studying,gallaba2018noise} (\eg missing dependencies and network access) or to flaky tests~\cite{dong2020concurrency,bell2018deflaker,herzig2015empirically, lam2019root}.
Our industrial partner observed that brown builds make developers lose trust in the CI system. Whenever a build fails, instead of verifying if the code is actually faulty, they would force a manual rerun of the build just to see if the result changes. This increases the build activity on the integration pipeline unnecessarily and increases the integration time. 
%The build will fail even though the code change is valid, and if the build was rerun, it could change its result and pass. Those unreliable failed builds are referred to as Brown Builds.

Several approaches have attempted to predict whether a build is brown or safe, based on flaky test detection approaches~\cite{bell2018deflaker} or ML models taking build job traces as input~\cite{lampel2021life,olewicki2022towards}. Our industry partner developed a brown build detection approach based on one of the latter models.



\subsubsection{Data extraction}
Table~\ref{info_proj} describes the dataset for brown build detection used in this paper. 
The dataset is composed of three closed-source projects provided by our industrial partner and one open-source project (Project Brown\_OSS).
The Brown Failure Rate $\beta$ refers to the percentage of brown job failures across all job failures, including reruns of builds. The studied projects were chosen to have at least 3 years of data with a consistent build job activity over time (at least 1k jobs per week). The projects differ in languages used, number of jobs, and in brownness ratio. Project Brown\_OSS corresponds to the Graphviz project, a graph visualization software publicly available on GitLab. We chose this dataset since it has a non-trivial brown failure ratio of 13\% that falls %which is significant (higher than 1\%) and 
in between the other datasets' brown failure ratio.

For the four projects, the dataset extracted is composed of build logs and CI meta information such as the job's name, number, associated commit id, and the timestamp of its beginning. This data is extracted from GitLab\footnote{Gitlab: \url{https://about.gitlab.com/}}. We also compute additional features about the number of past reruns of the job and the number of commits since the last brown job. These features are used to include information about the CI job's context and the moment it was run. 

% \textbf{Preprocessing}

% The feature extraction was done following the steps of a previous work~\cite{olewicki2022towards}.
% The jobs' logs are first filtered to remove some unique vocabulary (\eg timestamp, job or commit sha, filenames, and special characters). Words are then gathered into features using N-gram (\ie series of words of size $N$). Then, a word-count transformation is applied for each $N$.

% % Each job is then represented as a vector of 
% The vectorization of the data is done using TF-IDF\footnote{TF-IDF package: \texttt{sklearn.feature\_extraction.tex.TfidfVectorizer}} and a feature selection approach\footnote{KBest package: \texttt{sklearn.feature\_selection.SelectKBest}} (K-Best feature selection which selects the $K$ best features to keep). Each hyper-parameter mentioned here was tweaked to obtain the best performance across the four projects.

\subsection{Just-in-time risk prediction}

\subsubsection{Description}

JIT risk prediction predicts the riskiness of a code change based on metrics related to the change, such as the number of lines added/ modified/ removed, number of files touched, developer's experience, etc.~\cite{kamei2012large}. The term ``just-in-time'' refers to the fact that the detection is done while reviewing the code change instead of right before releasing. This has the advantage that the code change is fresh in the developers' mind.
Research has focused on making the prediction explainable, offering mitigation techniques to the developers to improve their code change~\cite{shihab2012industrial}. Furthermore,researchers have explored both %approaches of JIT risk prediction have been shown to use 
tree-based models~\cite{nayrolles2018clever} and neural network models~\cite{qiao2019effort}.

In our industrial partner's implementation of this approach, different features are fed to an XGBoost-based model~\cite{chen2015xgboost}, using an ensemble approach for prediction~\cite{zhou2021ensemble}. Several XGBoost models are thus trained on the data and the average result is used for prediction.
The tool is currently used by almost all the game projects of our industrial partner as an analytics tool for developers on the riskiness of their code changes or, in certain cases, as a step to integration. In the latter case, riskiness must be lower than a certain threshold to enable the CI build process.%trigger the build-generation system. 


\subsubsection{Data extraction}

In this paper we study four different closed source projects of our industrial partner, see Table~\ref{risk:info_proj}.
In these data sets, a code change is labeled as risky if it is tagged as bug-introducing in a Jira ticket.
Since Jira uses the SZZ approach~\cite{da2016framework} to associate buggy changes with the bug introducing changes, the labeling can thus be delayed sometimes by several months, depending on the time needed for the bug to be introduced.

The features used for the risk prediction approach involve meta-information about the submitted code change. Table~\ref{risk:info_feat} describes these features, where ``approvers'' are a special kind of reviewers that decide  which code changes can be integrated in an upcoming game release. All code changes are reviewed by at least one reviewer. When nearing a release date, the reviewed code changes are approved by an approver to be integrated in the next release (or pushed to the next release).


==> tables/RQ0.tex <==

\begin{table*}[t]
    \centering
    \caption{Cross-validation performance of hyperparameter optimization for the MLP models for the brown build detection and JIT risk prediction use cases. (For brown build detection, the \textcolor{cyan}{\textbf{bold blue}} values show the best F1-score/G-Mean per project.)}
    \label{MLP_hyper_res}
    \begin{tabularx}{\textwidth}{|l|XXXXX|XXXXX|XXXXX|XXXXX|}
    % \begin{tabular}{|p{1.7cm}|
    %             llp{.2cm}p{.3cm}p{.4cm}|
    %             llp{.2cm}p{.3cm}p{.4cm}|
    %             llp{.2cm}p{.3cm}p{.4cm}|
    %             llp{.2cm}p{.3cm}p{.4cm}|}
    	\hline
    	\multirow{3}{*}{Model}
            & \multicolumn{5}{c|}{Project Brown\_1} 
    	& \multicolumn{5}{c|}{Project Brown\_2}
            & \multicolumn{5}{c|}{Project Brown\_3} 
    	& \multicolumn{5}{c|}{Project Brown\_OSS} \\ \cline{2-21}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Brown}&\multicolumn{1}{p{.2cm}|}{Safe}
    	\\
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}\\ 
    	\cline{1-21}
    AlwaysBrown&
            23&0&30&100&0&
		27&0&37&100&0&
		5&0&5&100&0&
		12&0&13&100&0\\
       XGBoost
            &62&73&55&72&75 
            &67&\textcolor{cyan}{\textbf{72}}&57&81&64 
            &36&60&35&38&96 
            &\textcolor{cyan}{\textbf{52}}&72&{47}&{57}&{91}\\
    MLP  &\textcolor{cyan}{\textbf{73}}&\textcolor{cyan}{\textbf{79}}&{64}&{85}&{73}
        &\textcolor{cyan}{\textbf{70}}&71&{66}&{75}&{67}
        &\textcolor{cyan}{\textbf{44}}&\textcolor{cyan}{\textbf{68}}&{35}&{61}&{75}
        &50&\textcolor{cyan}{\textbf{77}}&38&73&81\\
    \hline
     \hline
         \multirow{3}{*}{Model}& \multicolumn{5}{c|}{Project Risk\_1} 
         & \multicolumn{5}{c|}{Project Risk\_2} 
         & \multicolumn{5}{c|}{Project Risk\_3} 
         & \multicolumn{5}{c|}{Project Risk\_4} \\ \cline{2-21}
         &\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}
    	&\multicolumn{1}{l|}{\multirow{2}{*}{F1}}&\multicolumn{1}{l|}{\multirow{2}{*}{GM}}&\multicolumn{2}{c|}{Risky}&\multicolumn{1}{p{.2cm}|}{Safe}
    	\\
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}
    	&\multicolumn{1}{p{.2cm}|}{}&\multicolumn{1}{p{.2cm}|}{}&Pre&\multicolumn{1}{p{.2cm}|}{Rec}&\multicolumn{1}{p{.2cm}|}{Rec}\\ 
    	\cline{1-21}
    AlwaysRisky&
            19&0&24   &100&0&
		21&0&27   &100&0&
		19&0&24    &100&0&
		13&0&15   &100&0\\
    MLP  & 45&58& 67& 36& 93
        & 49&61& 63& 42& 90
        & 43&58& 63& 36& 93
        & 21&38& 38& 15& 98\\ 
        %     MLP(NEW) 
        % &  53   &  64   &  58   &  49   &  83
        % &  48   &  63   &  46   &  51   &  77
        % &  45   &  64   &  42   &  47   &  87
        % &  55   &  68   &  52   &  59   &  78\\
        %     MLP(FUTURE) 
        % &  36   &  51   &  50   &  28   &  92
        % &  46   &  61   &  43   &  50   &  76
        % &  38   &  55   &  37   &  39   &  78
        % &  30   &  62   &  21   &  51   &  75\\
    \hline
    \end{tabularx}

\end{table*}


==> tables/data_risk.tex <==
\begin{table}[t]
	\centering
	\caption{\label{risk:info_proj} Studied projects for Just-In-Time risk prediction. The Risk rate represents the percentage of risky commits.}
	
	\begin{tabularx}{.47\textwidth}{|c|X|X|X|X|}%{|c||p{1.cm}|r|p{1.4cm}|p{.4cm}||p{1.2cm}|r|r|p{1.cm}|p{1.8cm}|p{2cm}|}
		\hline
		\multirow{2}{*}{\textbf{Projects}}&\textbf{Period [years]}&\textbf{\#commits}&\textbf{\#risky- commits}&\textbf{Risky rate \textbf{($RR$)}}\\
		%&&&&\textbf{($RR$)}\\
		\hline
		Risk\_1&5&50k&12k&24\%\\
		Risk\_2&4&49k&13k&27\%\\
		Risk\_3&9&82k&20k&24\%\\
		Risk\_4&5&57k&9k&15\%\\
		\hline
	\end{tabularx}
\end{table}

